OMiCroN -- Oblique Multipass Hierarchy Creation while Navigating

Rendering large point clouds ordinarily requires building a hierarchical data structure for accessing the points that best represent the object for a given viewing frustum and level-of-detail. The building of such data structures frequently represents a large portion of the cost of the rendering pipeline both in terms of time and space complexity, especially when rendering is done for inspection purposes only. This problem has been addressed in the past by incremental construction approaches, but these either result in low quality hierarchies or in longer construction times. In this work we present OMiCroN -- Oblique Multipass Hierarchy Creation while Navigating -- which is the first algorithm capable of immediately displaying partial renders of the geometry, provided the cloud is made available sorted in Morton order. OMiCroN is fast, being capable of building the entire data structure in memory spending an amount of time that is comparable to that of just reading the cloud from disk. Thus, there is no need for storing an expensive hierarchy, nor for delaying the rendering until the whole hierarchy is read from disk. In fact, a pipeline coupling OMiCroN with an incremental sorting algorithm running in parallel can start rendering as soon as the first sorted prefix is produced, making this setup very convenient for streamed viewing.

==> teaser.tex <==
\centering
	\includegraphics[width=2.5cm,height=6.5cm]{figs/teaser-10s.png}\hspace{1cm}
	\includegraphics[width=2.5cm,height=6.5cm]{figs/teaser-60s.png} \hspace{1cm}
	\includegraphics[width=2.5cm,height=6.5cm]{figs/teaser-120s.png}\hspace{1cm}
	\includegraphics[width=2.5cm,height=6.5cm]{figs/teaser-180s.png}\hspace{1cm}
	\includegraphics[width=2.5cm,height=6.5cm]{figs/teaser-200s.png} \\
	10s \hspace{3.2cm} 60s \hspace{3cm}120s \hspace{3cm}180s \hspace{3cm}200s
\caption{Real-time frames of the David model with 469 million points while reading from disk and simultaneously creating a space index hierarchy. The camera remained fixed for illustration purposes, but it can also freely move around the model during the hierarchy construction.}
\label{fig:teaser}


==> trechosort.tex <==
In order to assess the actual delay from the moment the raw unsorted collection of points is available, and the moment where rendering actually starts, we must consider the sorting process in some depth. The simplest scenario consists of a separate sorting process that reads the whole collection, sorts it and either outputs the ordered collection onto disk or streams it to the OMiCroN application. In this case, the OMiCroN must wait at least for the whole collection to be read by the sorting application, and for the sort itself. In a more ellaborate setup, the sorting process might start the streaming as soon as a prefix of the sorted collection becomes available. For instance, the QuickSort algorithm naturally lends itself to this kind of behavior, since the partition smaller than the pivot can be processed before the other partition. This means that the total delay is reduced to the time taken to read the whole collection, plus a small delay for obtaining the first prefix. Indeed, in our experiments, streaming starts at around $1.05I$, where $I$ is the time spent in reading the whole collection. 
